A Complete Proof System for 1-Free Regular Expressions Modulo Bisimilarity

Robin Milner (1984) gave a sound proof system for bisimilarity of regular expressions interpreted as processes: Basic Process Algebra with unary Kleene star iteration, deadlock 0, successful termination 1, and a fixed-point rule. He asked whether this system is complete. Despite intensive research over the last 35 years, the problem is still open. This paper gives a partial positive answer to Milner's problem. We prove that the adaptation of Milner's system over the subclass of regular expressions that arises by dropping the constant 1, and by changing to binary Kleene star iteration is complete. The crucial tool we use is a graph structure property that guarantees expressibility of a process graph by a regular expression, and is preserved by going over from a process graph to its bisimulation collapse.

==> figs/.jle/history/fig-ex-extr--sol-vs-extrsol.tex <==
\begin{figure*}[t!]
  %
\begin{center}
  %
  \begin{equation*}
    %
    \scalebox{0.92}{$
    \begin{aligned}[c]
      \extrsolof{\acharthat}{\averti{0}} 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\defdby$}\,
      \stexpbit{\stexpzero}{(\stexpprod{\aact}{\extrsolof{\acharthat}{\averti{1}}})}
      \\ 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpprod{\aact}{\extrsolof{\acharthat}{\averti{1}}}
      \\ 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpprod{\aact}{\stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                                            {\stexpprod{\aact}{(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                                 {\stexpzero}}
      \\
      \extrsolof{\acharthat}{\averti{1}} 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\defdby$}\,
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\extrsoluntilof{\acharthat}{\averti{0}}{\averti{1}}}}
                          {\stexpprod{\aact}{\extrsoluntilof{\acharthat}{\averti{2}}{\averti{1}}})}}
               {\stexpzero}
      \\ 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                          {\stexpprod{\aact}{(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
               {\stexpzero}
      \\
      \extrsoluntilof{\acharthat}{\averti{0}}{\averti{1}}
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\defdby$}\,
      \stexpbit{\stexpzero}{\aact}
      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \aact
      \\
      \extrsoluntilof{\acharthat}{\averti{2}}{\averti{1}}
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\defdby$}\,
      \stexpbit{\stexpzero}{(\stexpsum{\bact}{\stexpprod{\bact}{\extrsoluntilof{\acharthat}{\averti{0}}{\averti{1}}}})}
      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpsum{\bact}{\stexpprod{\bact}{\aact}}
      \\
      \extrsolof{\acharthat}{\averti{2}}
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\defdby$}\,
      \stexpbit{\stexpzero}{(\stexpsum{\stexpprod{\bact}{\extrsolof{\acharthat}{\averti{1}}}}
                                      {\stexpprod{\bact}{\extrsolof{\acharthat}{\averti{0}}}})}
      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpsum{\stexpprod{\bact}{\extrsolof{\acharthat}{\averti{1}}}}
               {\stexpprod{\bact}{(\stexpprod{\aact}{\extrsolof{\acharthat}{\averti{1}}})}}
      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpprod{(\stexpsum{\bact}{\stexpprod{\bact}{\aact})}}
                {\extrsolof{\acharthat}{\averti{1}}}
      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpprod{(\stexpsum{\bact}{\stexpprod{\bact}{\aact})}}
                {(\stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                                      {\stexpprod{\aact}{(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                           {\stexpzero})}
    \end{aligned}$}
    %
    \hspace*{-9ex}
    %
    \begin{aligned}[c]
      \\[-4ex]
      \scalebox{1.1}{\input{figs/fig-lLEEw-ex-extraction}}
    \end{aligned}
    %
    \hspace*{0ex}
    %
    \scalebox{0.92}{$
    \begin{aligned}[c]
      \asol{\averti{0}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpprod{\aact}{\asol{\averti{1}}}
        \;\;\;\parbox[t]{\widthof{(use of `is provable solution')}}
                        {(${}^{\text{\scriptsize (sol)}}$ means 
                         \\[-0.5ex]\phantom{(}%
                         use of `is provable solution')}
      \\[0.75ex]
      \asol{\averti{1}}   
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{\asol{\averti{0}}}}
               {\stexpprod{\aact}{\asol{\averti{2}}}} 
      \\[-0.25ex] 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asol{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
                                            {\stexpprod{\bact}{\asol{\averti{0}}}})}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asol{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
                                            {\stexpprod{\bact}{(\stexpprod{\aact}{\asol{\averti{1}}})}})}}
      \\
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \stexpsum{\stexpprod{(\stexpsum{\stexpprod{\cact}{\aact}}
                                     {\stexpprod{\aact}  
                                                {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                          {\asol{\averti{1}}}}
               {\stexpzero}           
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~~~~~~~$\Downarrow$\text{~~applying $\RSPbit$}} 
      \\[-0.25ex]  
      \asol{\averti{1}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\seqin{\BBP}$~}\;
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                          {\stexpprod{\aact}
                                     {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
               {\stexpzero} 
      % \\[-0.25ex]
      %   & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~~~~~~~$\Downarrow$\phantom{\text{~~applying $\RSPbit$}}} 
      % \\[-0.25ex] 
      \\
      % \Rightarrow\; 
      % \asol{\averti{1}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \extrsolof{\acharthat}{\averti{1}}  \quad \text{(see in the derivation on the left)}
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~~~~~~~$\Downarrow$\phantom{\text{~~applying $\RSPbit$}}} 
      \\[-0.25ex]
      \asol{\averti{0}}
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpprod{\aact}{\asol{\averti{1}}}
        ~~\seqin{\BBP}~~
      \stexpprod{\aact}{\extrsolof{\acharthat}{\averti{1}}}
        ~~\seqinsol{\BBP}~~
      \extrsolof{\acharthat}{\averti{0}}
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~~~~~~~$\Downarrow$\phantom{\text{~~applying $\RSPbit$}}} 
      \\[-0.25ex]
      \asol{\averti{2}}
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
               {\stexpprod{\bact}{\asol{\averti{0}}}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \stexpsum{\stexpprod{\bact}{\extrsolof{\acharthat}{\averti{1}}}}
               {\stexpprod{\bact}{\extrsolof{\acharthat}{\averti{0}}}} ~~\eqinsol{\BBP}~~ \extrsolof{\acharthat}{\averti{2}}
    \end{aligned}$}
    %
  \end{equation*}     
  %      
  \vspace*{-1.75ex}
  %
  \caption{\label{fig:ex:extr::sol:vs:extrsol}%
           Left:
           the process of extracting the provable solution~$\sextrsolof{\acharthat}$ of a chart $\achart$ from an \protect\LLEEwitness~$\acharthat$ of $\achart$
           as in the middle.\vspace*{-0.25mm} 
           Right: 
           steps for showing that an arbitrary provable solution~$\sasol$ of $\achart$ 
           is \protect\provablyin{\BBP} equal to the extracted solution $\sextrsolof{\acharthat}$.%
           }
\end{center}
  %
\end{figure*}  

==> figs/.jle/history/fig-ex-extraction.tex <==
\begin{figure}[t!]
  %
%\begin{center}
  %
  \begin{equation*}
    \hspace*{-7.5ex}
    \begin{aligned}[c]
      \scalebox{1.3}{\input{figs/fig-lLEEw-ex-extraction}}
    \end{aligned}
    \hspace*{1ex}
    \begin{aligned}[c]
      \extrsolof{\acharthat_1}{\averti{0}} 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\syntequal$}\,
      \stexpbit{\stexpzero}{(\stexpprod{\aact}{\extrsolof{\acharthat_1}{\averti{1}}})}
      \\ 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpprod{\aact}{\stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                                            {\stexpprod{\aact}{(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                                 {\stexpzero}}
      \\
      \extrsolof{\acharthat_1}{\averti{1}} 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\syntequal$}\,
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\extrsoluntilof{\acharthat_1}{\averti{0}}{\averti{1}}}}
                          {\stexpprod{\aact}{\extrsoluntilof{\acharthat_1}{\averti{2}}{\averti{1}}})}}
               {\stexpzero}
      \\ 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                          {\stexpprod{\aact}{(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
               {\stexpzero}
      \\
      \extrsoluntilof{\acharthat_1}{\averti{0}}{\averti{1}}
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\syntequal$}\,
      \stexpbit{\stexpzero}{\aact}
      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \aact
      \\
      \extrsoluntilof{\acharthat_1}{\averti{2}}{\averti{1}}
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\syntequal$}\,
      \stexpbit{\stexpzero}{(\stexpsum{\bact}{\stexpprod{\bact}{\extrsoluntilof{\acharthat_1}{\averti{0}}{\averti{1}}}})}
      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpsum{\bact}{\stexpprod{\bact}{\aact}}
      \\
      \extrsolof{\acharthat_1}{\averti{2}}
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\syntequal$}\,
      \stexpbit{\stexpzero}{(\stexpsum{\stexpprod{\bact}{\extrsolof{\acharthat_1}{\averti{1}}}}
                                      {\stexpprod{\bact}{\extrsolof{\acharthat_1}{\averti{0}}}})}
      \\
%        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
%      \stexpsum{\stexpprod{\bact}{\extrsolof{\acharthat_1}{\averti{1}}}}
%               {\stexpprod{\bact}{\stexpprod{\aact}{\extrsolof{\acharthat_1}{\averti{1}}}}}
%      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpprod{(\stexpsum{\bact}{\stexpprod{\bact}{\aact})}}
                {\extrsolof{\acharthat_1}{\averti{1}}}
      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpprod{(\stexpsum{\bact}{\stexpprod{\bact}{\aact})}}
                {(\stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                                      {\stexpprod{\aact}{(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                           {\stexpzero})}
    \end{aligned}
    %
  \end{equation*}     
  %      
%\end{center}
    \vspace*{-2ex}
 % \caption{\label{fig:ex:extraction}%
 %          Example of extracting a provable solution~$\sextrsolof{\acharthat_1}$ from a LLEE-witness~$\acharthat_1$.
 %          }

  %
\end{figure}      

==> figs/.jle/history/fig-ex-sol-vs-extrsol.tex <==
\begin{figure*}[t]
  %
\begin{center}
  %
  \begin{equation*}
    \hspace*{-3ex}
    \begin{aligned}[c]
      \scalebox{1}{\input{figs/fig-lLEEw-ex-extraction}}
    \end{aligned}
    \hspace*{-2ex}
    \scalebox{0.9}{$
    \begin{aligned}[c]
      \asol{\averti{0}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpprod{\aact}{\asol{\averti{1}}}
        \;\;\;\text{(${}^{\text{\scriptsize (sol)}}$ means use of `provable solution')}
      \\[0.75ex]
      \asol{\averti{1}}   
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{\asol{\averti{0}}}}
               {\stexpprod{\aact}{\asol{\averti{2}}}} 
      \\[-0.25ex] 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asol{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
                                            {\stexpprod{\bact}{\asol{\averti{0}}}})}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asol{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
                                            {\stexpprod{\bact}{(\stexpprod{\aact}{\asol{\averti{1}}})}})}}
      \\
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \stexpsum{\stexpprod{(\stexpsum{\stexpprod{\cact}{\aact}}
                                     {\stexpprod{\aact}
                                                {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                          {\asol{\averti{1}}}}
               {\stexpzero}           
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~~~~~~~$\Downarrow$\text{~~applying $\RSPbit$}} 
      \\[-0.25ex]  
      \asol{\averti{1}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\seqin{\BBP}$~}\;
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                          {\stexpprod{\aact}
                                     {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
               {\stexpzero} 
      \\
      \Rightarrow\;
      \asol{\averti{1}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \extrsolof{\acharthati{1}}{\averti{1}} 
        \;\;\;\text{(see Ex.\ \ref{ex:provable})}
      \\[0.75ex]
      \Rightarrow\;
      \asol{\averti{0}}
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpprod{\aact}{\asol{\averti{1}}}
        ~~\seqin{\BBP}~~
      \stexpprod{\aact}{\extrsolof{\acharthati{1}}{\averti{1}}}
        ~~\seqinsol{\BBP}~~
      \extrsolof{\acharthati{1}}{\averti{0}}
      \\[0.75ex]
      \Rightarrow\;
      \asol{\averti{2}}
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
               {\stexpprod{\bact}{\asol{\averti{0}}}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \stexpsum{\stexpprod{\bact}{\extrsolof{\acharthati{1}}{\averti{1}}}}
               {\stexpprod{\bact}{\extrsolof{\acharthati{1}}{\averti{0}}}} ~~\eqinsol{\BBP}~~ \extrsolof{\acharthati{1}}{\averti{2}}
    \end{aligned}$}
    %
  \end{equation*}     
  %      
\end{center}
  %
\end{figure*}  

==> figs/.jle/history/fig-prf-prop-extrsol-vs-solution.tex <==
\begin{figure*}
  \begin{minipage}{\textwidth}
    \begin{proof}[Proof (of Prop.~\ref{prop:extrsol:vs:solution})]
      Let $\acharthat$ be a \LLEEwitness\ of a chart~$\achart$. Let $\sasol$ be a provable solution of $\achart$.  
      We have to show that $\asol{\bvert} \BBPeq \extrsolof{\acharthat}{\bvert}$ for all $\bvert\neq\tick$.
      %
      For this, let $\bvert \neq \tick$.   
      The derivation below \vspace*{-.4mm}is based on the set representation of transitions from $\bvert$ in $\acharthat$ 
      as formulated in the definition of $\extrsolof{\acharthat}{\bvert}$.
      The first derivation step uses that $\sasol$ is a provable solution of $\achart$ and axioms $(\commstexpsum)$, $(\assocstexpsum)$, and $(\idempotstexpsum)$,
      the second step uses Lem.~\ref{lem:prop:extrsol:vs:solution} in view of $\bvert \descendsinloopto \bverti{j}$ for $j=1,\ldots,n$, 
      and the third step uses axioms $(\distr)$, $(\assocstexpprod)$, and $(\neutralstexpsum)$.
      \begin{align*}
        \asol{\bvert}~
          & \;\parbox[t]{\widthof{$\eqin{\BBP}$}}{$\BBPeq$}\:
            \stexpsum{
              \Bigl(
                \stexpsum{
                  \Bigl(
                    \sum_{i=1}^{m}
                      \stexpprod{\aacti{i}}{\asol{\bvert}}
                  \Bigr)
                          }{         
                  \Bigl(
                    \sum_{j=1}^{n}
                      \stexpprod{\bacti{j}}
                                {\asol{\bverti{j}}}
                  \Bigr)
                            }   
              \Bigr)
                      }{
              \Bigr(           
                \stexpsum{          
                  \Bigl(
                    \sum_{i=1}^{p}
                      \cacti{i}
                  \Bigr) 
                          }{
                  \Bigl(
                    \sum_{j=1}^{q}
                      \stexpprod{\dacti{j}}{\asol{\cverti{j}}}
                  \Bigr)
                            }
              \Bigr)
                         }          
            \\
          & \;\parbox[t]{\widthof{$\eqin{\BBP}$}}{$\BBPeq$}\:
            \stexpsum{
              \Bigl(
                \stexpsum{
                  \Bigl(
                    \sum_{i=1}^{m}
                      \stexpprod{\aacti{i}}{\asol{\bvert}}
                  \Bigr)
                          }{         
                  \Bigl(
                    \sum_{j=1}^{n}
                      \stexpprod{\bacti{j}}
                                {\bigl(
                                   \stexpprod{\extrsoluntilof{\acharthat}{\bverti{j}}{\bvert}}
                                             {\asol{\bvert}}
                                 \bigr)}             
                  \Bigr)
                            }   
              \Bigr)
                      }{
              \Bigr(           
                \stexpsum{          
                  \Bigl(
                    \sum_{i=1}^{p}
                      \cacti{i}
                  \Bigr) 
                          }{
                  \Bigl(
                    \sum_{j=1}^{q}
                      \stexpprod{\dacti{j}}{\asol{\cverti{j}}}
                  \Bigr)
                            }
              \Bigr)
                         }          
            \\
          & \;\parbox[t]{\widthof{$\eqin{\BBP}$}}{$\BBPeq$}\:
            \stexpsum{
              \stexpprod{
                \Bigl(
                  \stexpsum{
                    \Bigl(
                      \sum_{i=1}^{m}
                        \aacti{i}
                    \Bigr)
                            }{         
                    \Bigl(
                      \sum_{j=1}^{n}
                          \bigl(
                            \stexpprod{\bacti{j}}
                                      {\extrsoluntilof{\acharthat}{\bverti{j}}{\bvert}}
                          \bigr)
                    \Bigr)
                              }   
                \Bigr)
                       }{\asol{\bvert}}
                      }{
              \Bigr(           
                \stexpsum{          
                  \Bigl(
                    \sum_{i=1}^{p}
                      \cacti{i}
                  \Bigr) 
                          }{
                  \Bigl(
                    \sum_{j=1}^{q}
                      \stexpprod{\dacti{j}}{\asol{\cverti{j}}}
                  \Bigr)
                            }
              \Bigr)
                         } 
      \end{align*}  
      In view of this derived provable equality for $\asol{\bvert}$,
      we can now apply the rule $\RSPbit$ in order to obtain:
      \begin{align*}
        \asol{\bvert}~
          & \;\parbox[t]{\widthof{$\eqin{\BBP}$}}{$\BBPeq$}\:
            \Bigl(
              \stexpsum{
                \Bigl(
                  \sum_{i=1}^{m}
                    \aacti{i}
                \Bigr)
                        }{         
                \Bigl(
                  \sum_{j=1}^{n}
                        \stexpprod{\bacti{j}}
                                  {\extrsoluntilof{\acharthat}{\bverti{j}}{\bvert}}
                \Bigr)
                          }
                \Bigr)^{\sstexpbit}\hspace*{-1pt} 
                \Bigl(
                  \stexpsum{         
                    \Bigl(
                      \sum_{i=1}^{p}
                        \cacti{i}
                    \Bigr) 
                            }{
                    \Bigl(
                      \sum_{j=1}^{q}
                        \stexpprod{\dacti{j}}
                                  {\extrsolof{\acharthat}{\cverti{j}}}
                    \Bigr)   }
                \Bigr)
          ~~\parbox[t]{\widthof{$\syntequal$}}{$\syntequal$}~~
            \extrsolof{\acharthat}{\bvert}
      \end{align*}
    In this last step we have used the definition of $\extrsolof{\acharthat}{\bvert}$.  
    \end{proof}
  \end{minipage}
  \caption{\label{fig:prf:prop:extrsol:vs:sol}%
           Proof of Prop.~\ref{prop:extrsol:vs:solution}.}
\end{figure*}  

==> figs/.jle/history/fig-prop-extrsol-vs-solution.tex <==
\begin{figure*}
  \begin{minipage}{\textwidth}
    \begin{proof}[Proof of Prop.~\ref{prop:extrsol:vs:solution}]
      Let $\acharthat$ be a \LLEEwitness\ of a chart~$\achart$. Let $\sasol$ be a provable solution of $\achart$.  
      We have to show that $\asol{\bvert} \BBPeq \extrsolof{\acharthat}{\bvert}$ for all $\bvert\neq\tick$.
   
      For this, let $\bvert \neq \tick$.   
      The derivation below \vspace*{-.4mm}is based on the set representation of transitions from $\bvert$ in $\acharthat$ 
      as formulated in the definition of $\extrsolof{\acharthat}{\bvert}$.
      The first derivation step uses that $\sasol$ is a provable solution of $\achart$ and axioms $(\commstexpsum)$, $(\assocstexpsum)$, and $(\idempotstexpsum)$,
      the second step on Lem.~\ref{lem:prop:extrsol:vs:solution} for as $\bvert \descendsinloopto \bverti{j}$ for $j=1,\ldots,m$, 
      and the third step on axioms $(\distr)$ and $(\neutralstexpsum)$.
      \begin{align*}
        \asol{\bvert}~
          & \;\parbox[t]{\widthof{$\eqin{\BBP}$}}{$\BBPeq$}\:
            \stexpsum{
              \Bigl(
                \stexpsum{
                  \Bigl(
                    \sum_{i=1}^{m}
                      \stexpprod{\aacti{i}}{\asol{\bvert}}
                  \Bigr)
                          }{         
                  \Bigl(
                    \sum_{j=1}^{n}
                      \stexpprod{\bacti{j}}
                                {\asol{\bverti{j}}}
                  \Bigr)
                            }   
              \Bigr)
                      }{
              \Bigr(           
                \stexpsum{          
                  \Bigl(
                    \sum_{i=1}^{p}
                      \cacti{i}
                  \Bigr) 
                          }{
                  \Bigl(
                    \sum_{j=1}^{q}
                      \stexpprod{\dacti{j}}{\asol{\cverti{j}}}
                  \Bigr)
                            }
              \Bigr)
                         }          
            \\[0.25ex]
          & \;\parbox[t]{\widthof{$\eqin{\BBP}$}}{$\BBPeq$}\:
            \stexpsum{
              \Bigl(
                \stexpsum{
                  \Bigl(
                    \sum_{i=1}^{m}
                      \stexpprod{\aacti{i}}{\asol{\bvert}}
                  \Bigr)
                          }{         
                  \Bigl(
                    \sum_{j=1}^{n}
                      \stexpprod{\bacti{j}}
                                {\bigl(
                                   \stexpprod{\extrsoluntilof{\acharthat}{\bverti{j}}{\bvert}}
                                             {\asol{\bvert}}
                                 \bigr)}             
                  \Bigr)
                            }   
              \Bigr)
                      }{
              \Bigr(           
                \stexpsum{          
                  \Bigl(
                    \sum_{i=1}^{p}
                      \cacti{i}
                  \Bigr) 
                          }{
                  \Bigl(
                    \sum_{j=1}^{q}
                      \stexpprod{\dacti{j}}{\asol{\cverti{j}}}
                  \Bigr)
                            }
              \Bigr)
                         }          
            \\[0.25ex]
          & \;\parbox[t]{\widthof{$\eqin{\BBP}$}}{$\BBPeq$}\:
            \stexpsum{
              \stexpprod{
                \Bigl(
                  \stexpsum{
                    \Bigl(
                      \sum_{i=1}^{m}
                        \aacti{i}
                    \Bigr)
                            }{         
                    \Bigl(
                      \sum_{j=1}^{n}
                          \bigl(
                            \stexpprod{\bacti{j}}
                                      {\extrsoluntilof{\acharthat}{\bverti{j}}{\bvert}}
                          \bigr)
                    \Bigr)
                              }   
                \Bigr)
                       }{\asol{\bvert}}
                      }{
              \Bigr(           
                \stexpsum{          
                  \Bigl(
                    \sum_{i=1}^{p}
                      \cacti{i}
                  \Bigr) 
                          }{
                  \Bigl(
                    \sum_{j=1}^{q}
                      \stexpprod{\dacti{j}}{\asol{\cverti{j}}}
                  \Bigr)
                            }
              \Bigr)
                         } 
      \end{align*}  
      In view of this derived equality for $\asol{\bvert}$,
      the rule $\RSPbit$ can be applied to obtain:
      \begin{align*}
        \asol{\bvert}~
          & \;\parbox[t]{\widthof{$\eqin{\BBP}$}}{$\BBPeq$}\:
            \Bigl(
              \stexpsum{
                \Bigl(
                  \sum_{i=1}^{m}
                    \aacti{i}
                \Bigr)
                        }{         
                \Bigl(
                  \sum_{j=1}^{n}
                        \stexpprod{\bacti{j}}
                                  {\extrsoluntilof{\acharthat}{\bverti{j}}{\bvert}}
                \Bigr)
                          }
                \Bigr)^{\sstexpbit}\hspace*{-1pt} 
                \Bigl(
                  \stexpsum{         
                    \Bigl(
                      \sum_{i=1}^{p}
                        \cacti{i}
                    \Bigr) 
                            }{
                    \Bigl(
                      \sum_{j=1}^{q}
                        \stexpprod{\dacti{j}}
                                  {\extrsolof{\acharthat}{\cverti{j}}}
                    \Bigr)   }
                \Bigr)
          ~~\parbox[t]{\widthof{$\syntequal$}}{$\syntequal$}~~
            \extrsolof{\acharthat}{\bvert}
      \end{align*}
    In this last step we have used the definition of $\extrsolof{\acharthat}{\bvert}$.  
    \end{proof}
  \end{minipage}
  \caption{\label{fig:prf:prop:extrsol:vs:sol}%
           Proof of Prop.~\ref{prop:extrsol:vs:solution}.}
\end{figure*}  

==> figs/fig-ex-extr/.jle/history/sol-vs-extrsol.tex <==
\begin{figure*}[t]
  %
\begin{center}
  %
  \begin{equation*}
    \hspace*{-3ex}
    \begin{aligned}[c]
      \scalebox{1}{\input{figs/fig-lLEEw-ex-extraction}}
    \end{aligned}
    \hspace*{-2ex}
    \scalebox{0.9}{$
    \begin{aligned}[c]
      \asol{\averti{0}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpprod{\aact}{\asol{\averti{1}}}
        \;\;\;\text{(${}^{\text{\scriptsize (sol)}}$ means use of `provable solution')}
      \\[0.75ex]
      \asol{\averti{1}}   
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{\asol{\averti{0}}}}
               {\stexpprod{\aact}{\asol{\averti{2}}}} 
      \\[-0.25ex] 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asol{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
                                            {\stexpprod{\bact}{\asol{\averti{0}}}})}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asol{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
                                            {\stexpprod{\bact}{(\stexpprod{\aact}{\asol{\averti{1}}})}})}}
      \\
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \stexpsum{\stexpprod{(\stexpsum{\stexpprod{\cact}{\aact}}
                                     {\stexpprod{\aact}
                                                {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                          {\asol{\averti{1}}}}
               {\stexpzero}           
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~~~~~~~$\Downarrow$\text{~~applying $\RSPbit$}} 
      \\[-0.25ex]  
      \asol{\averti{1}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\seqin{\BBP}$~}\;
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                          {\stexpprod{\aact}
                                     {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
               {\stexpzero} 
      \\
      \Rightarrow\;
      \asol{\averti{1}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \extrsolof{\acharthati{1}}{\averti{1}} 
        \;\;\;\text{(see Ex.\ \ref{ex:provable})}
      \\[0.75ex]
      \Rightarrow\;
      \asol{\averti{0}}
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpprod{\aact}{\asol{\averti{1}}}
        ~~\seqin{\BBP}~~
      \stexpprod{\aact}{\extrsolof{\acharthati{1}}{\averti{1}}}
        ~~\seqinsol{\BBP}~~
      \extrsolof{\acharthati{1}}{\averti{0}}
      \\[0.75ex]
      \Rightarrow\;
      \asol{\averti{2}}
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
               {\stexpprod{\bact}{\asol{\averti{0}}}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \stexpsum{\stexpprod{\bact}{\extrsolof{\acharthati{1}}{\averti{1}}}}
               {\stexpprod{\bact}{\extrsolof{\acharthati{1}}{\averti{0}}}} ~~\eqinsol{\BBP}~~ \extrsolof{\acharthati{1}}{\averti{2}}
    \end{aligned}$}
    %
  \end{equation*}     
  %      
\end{center}
  %
\end{figure*}  

==> figs/fig-ex-extr/sol-vs-extrsol.tex <==
\begin{figure*}[t]
  %
\begin{center}
  %
  \begin{equation*}
    \hspace*{-3ex}
    \begin{aligned}[c]
      \scalebox{1}{\input{figs/fig-lLEEw-ex-extraction}}
    \end{aligned}
    \hspace*{-2ex}
    \scalebox{0.9}{$
    \begin{aligned}[c]
      \asol{\averti{0}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpprod{\aact}{\asol{\averti{1}}}
        \;\;\;\text{(${}^{\text{\scriptsize (sol)}}$ means use of `provable solution')}
      \\[0.75ex]
      \asol{\averti{1}}   
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{\asol{\averti{0}}}}
               {\stexpprod{\aact}{\asol{\averti{2}}}} 
      \\[-0.25ex] 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asol{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
                                            {\stexpprod{\bact}{\asol{\averti{0}}}})}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asol{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
                                            {\stexpprod{\bact}{(\stexpprod{\aact}{\asol{\averti{1}}})}})}}
      \\
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \stexpsum{\stexpprod{(\stexpsum{\stexpprod{\cact}{\aact}}
                                     {\stexpprod{\aact}
                                                {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                          {\asol{\averti{1}}}}
               {\stexpzero}           
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~~~~~~~$\Downarrow$\text{~~applying $\RSPbit$}} 
      \\[-0.25ex]  
      \asol{\averti{1}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\seqin{\BBP}$~}\;
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                          {\stexpprod{\aact}
                                     {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
               {\stexpzero} 
      \\
      \Rightarrow\;
      \asol{\averti{1}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \extrsolof{\acharthati{1}}{\averti{1}} 
        \;\;\;\text{(see Ex.\ \ref{ex:provable})}
      \\[0.75ex]
      \Rightarrow\;
      \asol{\averti{0}}
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpprod{\aact}{\asol{\averti{1}}}
        ~~\seqin{\BBP}~~
      \stexpprod{\aact}{\extrsolof{\acharthati{1}}{\averti{1}}}
        ~~\seqinsol{\BBP}~~
      \extrsolof{\acharthati{1}}{\averti{0}}
      \\[0.75ex]
      \Rightarrow\;
      \asol{\averti{2}}
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
               {\stexpprod{\bact}{\asol{\averti{0}}}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \stexpsum{\stexpprod{\bact}{\extrsolof{\acharthati{1}}{\averti{1}}}}
               {\stexpprod{\bact}{\extrsolof{\acharthati{1}}{\averti{0}}}} ~~\eqinsol{\BBP}~~ \extrsolof{\acharthati{1}}{\averti{2}}
    \end{aligned}$}
    %
  \end{equation*}     
  %      
\end{center}
  %
\end{figure*}  

==> figs/fig-ex-extraction.tex <==
\begin{figure}[t!]
  %
%\begin{center}
  %
  \begin{equation*}
    \hspace*{-7.5ex}
    \begin{aligned}[c]
      \scalebox{1.3}{\input{figs/fig-lLEEw-ex-extraction}}
    \end{aligned}
    \hspace*{1ex}
    \begin{aligned}[c]
      \extrsolof{\acharthat_1}{\averti{0}} 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\syntequal$}\,
      \stexpbit{\stexpzero}{(\stexpprod{\aact}{\extrsolof{\acharthat_1}{\averti{1}}})}
      \\ 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpprod{\aact}{\stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                                            {\stexpprod{\aact}{(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                                 {\stexpzero}}
      \\
      \extrsolof{\acharthat_1}{\averti{1}} 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\syntequal$}\,
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\extrsoluntilof{\acharthat_1}{\averti{0}}{\averti{1}}}}
                          {\stexpprod{\aact}{\extrsoluntilof{\acharthat_1}{\averti{2}}{\averti{1}}})}}
               {\stexpzero}
      \\ 
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                          {\stexpprod{\aact}{(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
               {\stexpzero}
      \\
      \extrsoluntilof{\acharthat_1}{\averti{0}}{\averti{1}}
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\syntequal$}\,
      \stexpbit{\stexpzero}{\aact}
      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \aact
      \\
      \extrsoluntilof{\acharthat_1}{\averti{2}}{\averti{1}}
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\syntequal$}\,
      \stexpbit{\stexpzero}{(\stexpsum{\bact}{\stexpprod{\bact}{\extrsoluntilof{\acharthat_1}{\averti{0}}{\averti{1}}}})}
      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpsum{\bact}{\stexpprod{\bact}{\aact}}
      \\
      \extrsolof{\acharthat_1}{\averti{2}}
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\syntequal$}\,
      \stexpbit{\stexpzero}{(\stexpsum{\stexpprod{\bact}{\extrsolof{\acharthat_1}{\averti{1}}}}
                                      {\stexpprod{\bact}{\extrsolof{\acharthat_1}{\averti{0}}}})}
      \\
%        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
%      \stexpsum{\stexpprod{\bact}{\extrsolof{\acharthat_1}{\averti{1}}}}
%               {\stexpprod{\bact}{\stexpprod{\aact}{\extrsolof{\acharthat_1}{\averti{1}}}}}
%      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpprod{(\stexpsum{\bact}{\stexpprod{\bact}{\aact})}}
                {\extrsolof{\acharthat_1}{\averti{1}}}
      \\
        & \;\parbox[t]{\widthof{~~$\BBPeq$~~}}{~~$\BBPeq$~~}\,
      \stexpprod{(\stexpsum{\bact}{\stexpprod{\bact}{\aact})}}
                {(\stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                                      {\stexpprod{\aact}{(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                           {\stexpzero})}
    \end{aligned}
    %
  \end{equation*}     
  %      
%\end{center}
    \vspace*{-2ex}
 % \caption{\label{fig:ex:extraction}%
 %          Example of extracting a provable solution~$\sextrsolof{\acharthat_1}$ from a LLEE-witness~$\acharthat_1$.
 %          }

  %
\end{figure}      

==> figs/fig-ex-sol-vs-extrsol-old.tex <==
%\begin{figure}[tbp]
  %
\begin{center}
  %
  \begin{equation*}
    \hspace*{-7.5ex}
    \begin{aligned}[c]
      \scalebox{1.3}{\input{figs/fig-lLEEw-ex-extraction}}
    \end{aligned}
    \hspace*{-1ex}
    \begin{aligned}[c]
      \asol{\averti{0}} 
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpprod{\aact}{\asol{\averti{1}}}
        \;\;\;\text{(${}^{\text{\scriptsize (sol)}}$ means use of `provable solution')}
        %\;\;\;\text{$(\seqinsol{\BBP}$ means use of `is \BBP-solution')}
      \\[0.75ex]
      \asol{\averti{1}}   
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpsum{\stexpprod{\cact}{\asol{\averti{0}}}}
               {\stexpprod{\aact}{\asol{\averti{2}}}} 
      \\[-0.25ex] 
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asol{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
                                            {\stexpprod{\bact}{\asol{\averti{0}}}})}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asol{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
                                            {\stexpprod{\bact}{(\stexpprod{\aact}{\asol{\averti{1}}})}})}}
      \\
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqin{\BBP}$}\;
      \stexpsum{\stexpprod{(\stexpsum{\stexpprod{\cact}{\aact}}
                                     {\stexpprod{\aact}
                                                {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                          {\asol{\averti{1}}}}
               {\stexpzero}           
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\Downarrow$\text{ applying $\RSPbit$}} 
      \\[-0.75ex]  
      \asol{\averti{1}} 
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\seqin{\BBP}$}\;
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                          {\stexpprod{\aact}
                                     {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
               {\stexpzero} 
      %  \,\eqin{\BBP}\,
      % \extrsolof{\acharthat}{\averti{1}}           
      %\\
      %  & \;\parbox[t]{\widthof{$\seqinsol{\BBP}$}}{$\Downarrow$}\;
      \\
      \Rightarrow\;
      \asol{\averti{1}} 
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqin{\BBP}$}\;
      \extrsolof{\acharthati{1}}{\averti{1}} 
        \;\;\;\text{(see extraction example)}
      \\[0.75ex]
      \Rightarrow\;
      \asol{\averti{0}}
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpprod{\aact}{\asol{\averti{1}}}
        \,\seqin{\BBP}\,
      \stexpprod{\aact}{\extrsolof{\acharthati{1}}{\averti{1}}}
        \,\seqinsol{\BBP}\,
      \extrsolof{\acharthati{1}}{\averti{0}}
      \\[0.75ex]
      \Rightarrow\;
      \asol{\averti{2}}
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
               {\stexpprod{\bact}{\asol{\averti{0}}}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqin{\BBP}$}\;
      \stexpsum{\stexpprod{\bact}{\extrsolof{\acharthati{1}}{\averti{1}}}}
               {\stexpprod{\bact}{\extrsolof{\acharthati{1}}{\averti{0}}}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \extrsolof{\acharthati{1}}{\averti{2}}               
    \end{aligned}
    %
  \end{equation*}     
  %      
\end{center}
%    \vspace*{-2ex}
%  \caption{\label{fig:ex:sol:vs:extrsol}%
%           Example for showing 
%           that a \protect\provablein{\BBP} solution~$\sasol$
%           on a chart with a LLEE-witness~$\acharthat$ is \protect\provablyin{\BBP} equal 
%           to the solution~$\sextrsolof{\acharthat}$ extracted from $\acharthat$, see earlier example %Figure~\ref{fig:ex:extraction}.
           % By $\seqinsol{\BBP}$ we indicate a use of the defining property of a \protect\provablein{\BBP} solution.
  %         }
  %
%\end{figure}      

==> figs/fig-ex-sol-vs-extrsol.tex <==
%\begin{figure}[tbp]
  %
\begin{center}
  %
  \begin{equation*}
    \hspace*{-3ex}
    \begin{aligned}[c]
      \scalebox{1.1}{\input{figs/fig-lLEEw-ex-extraction}}
    \end{aligned}
    \hspace*{-2ex}
    \begin{aligned}[c]
      \asol{\averti{0}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpprod{\aact}{\asol{\averti{1}}}
        \;\;\;\text{(${}^{\text{\scriptsize (sol)}}$ means use of `provable solution')}
      \\[0.75ex]
      \asol{\averti{1}}   
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{\asol{\averti{0}}}}
               {\stexpprod{\aact}{\asol{\averti{2}}}} 
      \\[-0.25ex] 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asol{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
                                            {\stexpprod{\bact}{\asol{\averti{0}}}})}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asol{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
                                            {\stexpprod{\bact}{(\stexpprod{\aact}{\asol{\averti{1}}})}})}}
      \\
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \stexpsum{\stexpprod{(\stexpsum{\stexpprod{\cact}{\aact}}
                                     {\stexpprod{\aact}
                                                {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                          {\asol{\averti{1}}}}
               {\stexpzero}           
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~~~~~~~$\Downarrow$\text{~~applying $\RSPbit$}} 
      \\[-0.25ex]  
      \asol{\averti{1}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\seqin{\BBP}$~}\;
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                          {\stexpprod{\aact}
                                     {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
               {\stexpzero} 
      \\
      \Rightarrow\;
      \asol{\averti{1}} 
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \extrsolof{\acharthati{1}}{\averti{1}} 
        \;\;\;\text{(see Ex.\ \ref{ex:provable})}
      \\[0.75ex]
      \Rightarrow\;
      \asol{\averti{0}}
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpprod{\aact}{\asol{\averti{1}}}
        ~~\seqin{\BBP}~~
      \stexpprod{\aact}{\extrsolof{\acharthati{1}}{\averti{1}}}
        ~~\seqinsol{\BBP}~~
      \extrsolof{\acharthati{1}}{\averti{0}}
      \\[0.75ex]
      \Rightarrow\;
      \asol{\averti{2}}
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqinsol{\BBP}$~}\;
      \stexpsum{\stexpprod{\bact}{\asol{\averti{1}}}}
               {\stexpprod{\bact}{\asol{\averti{0}}}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{~$\eqinsol{\BBP}$~}}{~$\eqin{\BBP}$~}\;
      \stexpsum{\stexpprod{\bact}{\extrsolof{\acharthati{1}}{\averti{1}}}}
               {\stexpprod{\bact}{\extrsolof{\acharthati{1}}{\averti{0}}}} ~~\eqinsol{\BBP}~~ \extrsolof{\acharthati{1}}{\averti{2}}
    \end{aligned}
    %
  \end{equation*}     
  %      
\end{center}

==> figs/fig-ex-unique-solvability.tex <==
\begin{figure}[tbp]
  %
\begin{center}
  %
  \begin{equation*}
    \hspace*{-7.5ex}
    \begin{aligned}[c]
      \scalebox{1.3}{\input{figs/fig-lLEEw-ex-extraction}}
    \end{aligned}
    \hspace*{-1.75ex}
    \begin{aligned}[c]
      \asoli{{1}/{2}}{\averti{0}} 
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpprod{\aact}{\asoli{{1}/{2}}{\averti{1}}}
        \;\;\;\text{(${}^{\text{\scriptsize (sol)}}$ means use of `is \BBP-solution')}
      \\[0.75ex]
      \asoli{{1}/{2}}{\averti{1}} 
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpsum{\stexpprod{\cact}{\asoli{{1}/{2}}{\averti{0}}}}
               {\stexpprod{\aact}{\asoli{{1}/{2}}{\averti{2}}}} 
      \\[-0.25ex] 
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asoli{{1}/{2}}{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asoli{{1}/{2}}{\averti{1}}}}
                                            {\stexpprod{\bact}{\asoli{{1}/{2}}{\averti{0}}}})}}
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpsum{\stexpprod{\cact}{(\stexpprod{\aact}{\asoli{{1}/{2}}{\averti{1}}})}}
               {\stexpprod{\aact}{(\stexpsum{\stexpprod{\bact}{\asoli{{1}/{2}}{\averti{1}}}}
                                            {\stexpprod{\bact}{(\stexpprod{\aact}{\asoli{{1}/{2}}{\averti{1}}})}})}}
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpsum{\stexpprod{(\stexpsum{\stexpprod{\cact}{\aact}}
                                     {\stexpprod{\aact}
                                                {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
                          {\asoli{1/2}{\averti{1}}}}
               {\stexpzero}           
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\Downarrow$\text{ applying $\RSPbit$}} 
      \\[-0.75ex]  
      \asoli{{1}/{2}}{\averti{1}} 
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpbit{(\stexpsum{\stexpprod{\cact}{\aact}}
                          {\stexpprod{\aact}
                                     {(\stexpsum{\bact}{\stexpprod{\bact}{\aact}})}})}
               {\stexpzero}   
      \\[-0.25ex]
      \Rightarrow\;
      \asoli{1}{\averti{1}} 
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \asoli{2}{\averti{1}}
      \\[0.5ex]
      \Rightarrow\;
      \asoli{1}{\averti{0}}
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpprod{\aact}{\asoli{1}{\averti{1}}}
        \,\eqin{\BBP}\,
      \stexpprod{\aact}{\asoli{2}{\averti{1}}}
        \,\eqinsol{\BBP}\,
      \asoli{2}{\averti{0}}
      \\[0.5ex]
      \Rightarrow\;
      \asoli{1}{\averti{2}}
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \stexpsum{\stexpprod{\bact}{\asoli{1}{\averti{1}}}}
               {\stexpprod{\bact}{\asoli{1}{\averti{0}}}} 
      \\[-0.5ex]
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinphansol{\BBP}$}\;
      \stexpsum{\stexpprod{\bact}{\asoli{2}{\averti{1}}}}
               {\stexpprod{\bact}{\asoli{2}{\averti{0}}}} 
      \\[-0.25ex]
        & \;\parbox[t]{\widthof{$\eqinsol{\BBP}$}}{$\eqinsol{\BBP}$}\;
      \asoli{2}{\averti{2}}               
    \end{aligned}
    %
  \end{equation*}     
  %      
\end{center}
    \vspace*{-2ex}
  \caption{\label{fig:ex:unique:solvability}%
           Proving \protect\BBP-equality of two \protect\BBP-solutions $\sasoli{1}$ and $\sasoli{2}$ of a LLEE-chart.}
  %
\end{figure}      
